How Medical Crowdfunding Helps People? A Large-scale Case Study on Waterdrop Fundraising

While online medical crowdfunding achieved tremendous success, quantitative study about whether and how medical crowdfunding helps people remains little explored. In this paper, we empirically study how online medical crowdfunding helps people using more than 27, 000 fundraising cases in Waterdrop Fundraising, one of the most popular online medical crowdfunding platforms in China. We find that the amount of money obtained by fundraisers is broadly distributed, i.e., a majority of lowly donated cases coexist with a handful of very successful cases. We further investigate the factors that potentially correlate with the success of medical fundraising cases. Profile information of fundraising cases, e.g., geographic information of fundraisers, affects the donated amounts, since detailed description may increase the credibility of a fundraising case. One prominent finding lies in the effect of social network on the success of fundraising cases: the spread of fundraising information along social network is a key factor of fundraising success, and the social capital of fundraisers play an important role in fundraising. Finally, we conduct prediction of donations using machine learning models, verifying the effect of potential factors to the success of medical crowdfunding. Altogether, this work presents a data-driven view of medical fundraising on the web and opens a door to understanding medical crowdfunding.

==> 8-related-work.tex <==
\subsection{Crowdfunding Mechanism}
Crowdfunding is defined as an open call mostly through the Internet for the provision of financial resources by a group of individuals instead of professional parties either in the form of donations, in exchange for a future product, or exchange for some kind form of reward \cite{belleflamme2014crowdfunding, schwienbacher2010crowdfunding,gerber2013crowdfunding}. 
Crowdfunding typically contains three participating stakeholders: the project initiators who seek funding for their projects, the backers who are willing to back a specific project, and the matchmaking crowdfunding platforms acting as intermediaries \cite{gierczak2016crowdfunding, belleflamme2014crowdfunding}. 
Many researchers have discussed and studied the relationship between the three parts, their motivations, benefits, and risks \cite{gerber2013crowdfunding, haas2014empirical, belleflamme2014crowdfunding, gierczak2014all}.
The study on crowdfunding mechanism is increasingly gaining attention in several scientific fields, including economics, management, and social computing.

For social computing, researchers will focus on some phenomenons or some factors (\eg, donor retention \cite{althoff2015donor}, trust amid delays \cite{kim2017understanding}, credibility factors \cite{kim2016power} and so on) to analyze the crowdfunding mechanism.
Especially, much of the CSCW research on crowdfunding has looked at coordination between project creators and donors or potential donors \cite{solomon2015don}.
Gerber et al \cite{gerber2013crowdfunding} find that the fundraisers' motivations involves the desire to raise funds, expand awareness 34 of work, connect with others, gain approval, maintain control, and learn; and supporters' motivations include the desire to collect rewards, help others, support causes, and be part of a community.
Muller et al. studied the crowdfunding inside the enterprise for innovation and collaboration, geographical and organizational distances  \cite{muller2013crowdfunding, muller2014geographical}.
Except for motivations, the success of crowdfunding is another focus of researchers. 
A large number of studies analyze the factors that affect the success of crowdfunding cases and try to build some machine learning models that can predict the success probability of the case to provide better suggestions to fundraisers and platforms \cite{muller2016social, greenberg2014learning,etter2013launch, cheng2019success}.

However, the related crowdfunding studies are mainly about commercial crowdfunding which aimed at raising money for their own commercial ventures \cite{tanaka2016legitimacy}.
Philanthropic crowdfunding is a new kind of crowdfunding which is used by nonprofit organizations or individuals to raise money for informal and formal charities.
Tanaka et al. demonstrated that the legitimacy of a philanthropic crowdfunding campaign is a central concern for fundraisers \cite{tanaka2016legitimacy}.
For the medical crowdfunding, Kim et al. interviewed fifteen people involved in medical crowdfunding and found that support networks were larger than beneficiaries expected, with strangers offering support. 
Supporters offered not only monetary but also volunteering contributions including campaign creation, promotion, and external support \cite{kim2017not}.
This work is nearly for our research findings. 
We also find that the social networks not only provide donations but also some volunteering contributions(\eg verifying and sharing). 

\subsection{Popularity prediction}
% 
% 伴随这web2.0的发展，各种各样的社会媒体快速兴起，有关社会媒体信息传播的研究引起研究人员的广泛关注。
% 过去的流行度预测主要集中于微博，xxxxx等媒体。方法建模上主要包括事前预测和早期预测。研究人员从各种不同的纬度对流行度预测进行了建模，包括。
% 但是关于众筹的信息传播相关的研究较少，这篇文章将一些过去成功应用到微博等常见下的模型和方法迁移到关于筹款和转发的预测上。希望能够更好的理解和建模在互联网疾病众筹常见下的流行度预测。
The popularity of web content is the amount of attention that web content \cite{gao2019taxonomy, tatar2014survey}. 
In certain instances, a photo, link, or other pieces of information may get reshared multiple times: a user shares the content with his friends, several of these friends share it with their respective friends, and a cascade of resharing can develop, potentially reaching a large number of people \cite{cheng2014can}.
Some studies choose to predict popularity at the time of posting when the information diffusion has not happened. 
However, a more widely adopted approach includes peeking into the initial stages of diffusion, suggesting that early patterns are tightly connected to the eventual fate of the item \cite{gao2019taxonomy}. 
According to the timing of prediction, the prediction of web content in online social networks can be divided into two types: ex-ante prediction and early prediction \cite{hofman2017prediction}.
The ex-ante prediction uses only information available before a given cascade. 
The early prediction will observe the progression of a cascade for some time before making a prediction \cite{hofman2017prediction}.
Many researchers point out that temporal features are a key predictor and generalize fairly compare to network structure features and content features \cite{shulman2016predictability, szabo2010predicting, pinto2013using, yu2015micro}.
The particular types of popularity prediction involves tweet/microblogs \cite{gao2019taxonomy, martin2016exploring, bao2015modeling, bao2013popularity}, images \cite{zhang2018user}, videos \cite{rizoiu2017expecting}, recipes \cite{sanjo2017recipe}, academic papers \cite{shen2014modeling} and so on.
% The main methods for popularity prediction include feature-based extraction models, point process-based modeling, and deep learning-based methods.
% Feature based extraction models usually manually extract valuable features for specific platforms or datasets(\ie Youtube, Twitter, Weibo). 
% These features usually include user features \cite{gao2019taxonomy, bakshy2011everyone}, content features \cite{tsur2012s, petrovic2011rt}, and time series features \cite{pinto2013using,szabo2010predicting} and structural characteristics \cite{shulman2016predictability,bao2013popularity, gao2014effective}.
% Point process-based modeling considers information diffusion as an arrival process and uses different functions to model the rate function. 
% These functions include Reinforced Poisson Process \cite{shen2014modeling, gao2014effective} and Self-exciting Process \cite{zhao2015seismic,rizoiu2017expecting,bao2015modeling}.
% Deep learning-based methods mainly use different neural networks to model the features instead of feature engineering. 
% Different neural networks model different types of data. 
% Common deep learning models include Convolutional Neural Network(CNN) \cite{zhang2018user}, Recurrent Neural Network(RNN) \cite{wang2018learning}, Temporal Convolutional Network(TCN) \cite{shao2019temporal} and Graph Neural Network(GNN) \cite{cao2020coupledgnn, qiu2018deepinf}.

In the context of medical crowdfunding, information diffusion is an important mechanism. 
Some researches on popularity prediction can help us better analyze, model, and predict medical crowdfunding donations.
% 基于特征提取的消息流行度预测模型，通常会为特定的平台或数据集
% 分为事前预测和早期预测



